Algorithm-driven Advances for Scientific CT Instruments: From Model-based to Deep Learning-based Approaches

Multi-scale 3D characterization is widely used by materials scientists to further their understanding of the relationships between microscopic structure and macroscopic function. Scientific computed tomography (CT) instruments are one of the most popular choices for 3D non-destructive characterization of materials at length scales ranging from the angstrom-scale to the micron-scale. These instruments typically have a source of radiation that interacts with the sample to be studied and a detector assembly to capture the result of this interaction. A collection of such high-resolution measurements are made by re-orienting the sample which is mounted on a specially designed stage/holder after which reconstruction algorithms are used to produce the final 3D volume of interest. The end goal of scientific CT scans include determining the morphology,chemical composition or dynamic behavior of materials when subjected to external stimuli. In this article, we will present an overview of recent advances in reconstruction algorithms that have enabled significant improvements in the performance of scientific CT instruments - enabling faster, more accurate and novel imaging capabilities. In the first part, we will focus on model-based image reconstruction algorithms that formulate the inversion as solving a high-dimensional optimization problem involving a data-fidelity term and a regularization term. In the last part of the article, we will present an overview of recent approaches using deep-learning based algorithms for improving scientific CT instruments.

==> bio.tex <==
\normalsize{\textbf{S. V. Venkatakrishnan} received the Ph.D. degree from the School of Electrical and Computer Engineering at Purdue University in 2014.
%with a thesis focused on the development of model-based reconstruction algorithms for nano-scale and micro-scale imaging. 
%He was subsequently a post-doctoral fellow at Lawrence Berkeley National Laboratory where he developed reconstruction algorithms for X-ray scattering and tomography. 
He is currently a R\&D Staff member at the Multimodal Sensor Analytics group at Oak Ridge National Laboratory developing computational imaging algorithms in support of the lab’s efforts in ultrasound, X-ray, electron and neutron-based systems. 
His research interests include Computational Imaging, Inverse Problems and Machine Learning. 
He was awarded a Presidential Scholar Award at the Microscopy and Microanalysis conference (2014), and the Eugene P. Wigner Distinguished Staff Fellowship at Oak Ridge National Lab (2016-2019). 
He is also a recipient of the SIAM SIAG/IS Best Paper Award (2020). 
Dr. Venkatakrishnan is a senior member of the IEEE, a member of the IEEE Computational Imaging Technical Committee and an Associate Editor of the IEEE Trans. On Computational Imaging.
}

\normalsize{\textbf{K. Aditya Mohan} received the Ph.D. degree from the School of Electrical and Computer Engineering at Purdue University in 2017. He is currently a signal and image processing engineer in the Computational Engineering Division (CED) at Lawrence Livermore National Lab (LLNL). His research involves solving inverse problems in computational imaging using numerical optimization and machine learning. His current research interests are in computational imaging, inverse problems, statistical signal processing, optimization, and deep learning.}  
 
 \normalsize{\textbf{Amir Koushyar Ziabari} is an R\&D staff scientist in the Multimodal Sensor Analytics group at Oak Ridge National Laboratory (ORNL).  Before joining ORNL, Dr. Ziabari was a Postdoc at Integrated Imaging group at the Department of Electrical and Computer Engineering (ECE) at the Purdue University. He also received his PhD from the department of ECE at Purdue University in August 2016. His research interests have been at the intersection of physics, signal processing and machine/deep learning, where he has used image/signal processing and machine learning ideas to explore multi-scale experimental physics phenomena. He is currently working on data analytics, data driven and physics-based image reconstruction and segmentation for advanced manufacturing (AM) in order to improve non-destructive evaluation (NDE) and the state-of-the-art in real time monitoring of the AM process.}
 
 \normalsize{\textbf{Charles A. Bouman} received a Ph.D. in electrical engineering from Princeton University. 
 He joined the faculty of Purdue University in 1989 where he is currently the Showalter Professor of Electrical and Computer Engineering and Biomedical Engineering.
Prof. Bouman's research is in the area of computational imaging and sensing where he is focused on the integration of signal processing, statistical modeling, physics, and computation to solve difficult sensing problems with applications in healthcare, material science, physics, chemistry, commercial and consumer imaging. 
Professor Bouman is a member of the National Academy of Inventors, a Fellow of the IEEE, a Fellow of the American Institute for Medical and Biological Engineering (AIMBE), a Fellow of the society for Imaging Science and Technology (IS\&T), a Fellow of the SPIE professional society. 
He is the recipient of the 2014 Electronic Imaging Scientist of the Year award, and the IS&T’s Raymond C. Bowman Award; and in 2020, his paper on Plug-and-Play Priors won the SIAM Imaging Science Best Paper Prize. He was previously the Editor-in-Chief for the IEEE Transactions on Image Processing; a Distinguished Lecturer for the IEEE Signal Processing Society; and a Vice President of Technical Activities for the IEEE Signal Processing Society, during which time he led the creation of the IEEE Transactions on Computational Imaging. 
%He has been an associate editor for the IEEE Transactions on Image Processing, the IEEE Transactions on Pattern Analysis and Machine Intelligence, and the SIAM Journal on Mathematical Imaging. He has also been a Vice President of Publications and a member of the Board of Directors for the IS&T Society, and he is the founder and Co-Chair of the SPIE/IS&T conference on Computational Imaging. 
}

==> front.tex <==
\begin{abstract}
Computed tomography (CT) instruments are widely used for 3D non-destructive characterization of materials from the nano-meter to the micron length scales. 
Despite of advances in various hardware components within scientific CT instruments, obtaining high quality images can be challenging because of the complicated nature of the physics of interaction between the source of radiation and the sample under study, noise in the measurement and the sparse/limited nature of the data dictated by experimental constraints. 
Recently, there has been a lot of progress in the development of novel reconstruction algorithms that have enabled high-quality images to be obtained from scientific CT instruments that are commonly used in the material sciences. 
In this article, we will present an overview of the development of two classes of algorithms - model-based image reconstruction and non-iterative deep-learning based reconstruction - that have enabled dramatic improvements in the resolution and throughput of a wide variety of instruments including electron, X-ray, and neutron CT systems. 
%Overall, the algorithms have expanded the capabilities of scientific CT instruments by enabling  improvements in resolution and throughput.  
\end{abstract}


==> summary.tex <==
\section*{Motivation and Significance}

%What is scientific CT; Why is it important for materials imaging
 Multi-scale 3D characterization is widely used by scientists to further their understanding of material behavior, to establish relationships between microscopic structure and macroscopic function, and eventually to enable them to engineer materials with sophisticated properties by manipulating matter at the sub-micron length scales. 
Scientific computed tomography (CT) instruments are widely used for 3D characterization at different length scales ranging from angstrom-scale imaging to sub-micron imaging using sophisticated instruments including electron microscopes \cite{saghi2012electron,ercius2015electron}, lab-based or synchrotron-based X-ray microscopes \cite{stock2008recent,singh20193d} and neutron-based instruments \cite{brenizer2013review,bilheux2015overview}. 
These instruments typically have a source of particles that interacts with the sample to be studied and a detector assembly to capture the result of this interaction. 
A collection of such measurements are made by re-orienting the sample, after which  \textit{reconstruction algorithms} are used to produce the final 3D volume of interest corresponding to the sample. 
The instruments used for scientific CT are often very expensive and are operated in facilities where multiple users share the instrument in order to make their measurements. 
As a result, unlike in medical CT, these instruments are not optimized for measuring a specific type of sample.
Furthermore, they are designed to be flexible in order for scientists to be able to modify the instruments to conduct studies of samples under varying environmental conditions.
In summary, scientific CT instruments are powerful and flexible tools that enable 3D characterization across multiple length scales and play a critical role in furthering our understanding of the structure-function relationships of various materials. 

%CT is carried out using electron, X-ray, neutron and optical instruments enabling characterization of materials from the atomic scale to the millimeter scale. 
While significant investments and advances have been made in developing various hardware components of scientific CT instruments, until recently there has been less focus on the development of reconstruction algorithms in order to deal with the various challenges encountered.  
The first generation of CT systems have typically relied on analytic algorithms to perform the 3D reconstructions because of their widespread availability and their low computational complexity. 
In fact, a cursory survey of the methods section of scientific publications that use CT as a part of their investigation, suggest that such analytic reconstruction algorithms are still the most popular choice for tomographic  reconstruction. 
However, the performance of these algorithms can be poor when dealing with non-linearities in the measurement induced by the unique nature of certain materials, the presence of high-levels of noise, and the limited number of measurements that can occur when one seeks to accelerate the acquisition to improve overall throughput or to enable high-resolution time-resolved 3D imaging of materials when they are subjected to external stimuli such as temperature or pressure. 
Thus, the reliance on the use of analytic reconstruction techniques in turn limits the characterization capability of scientific CT instruments, and has led to an inefficient usage of the instrument time by collecting large amounts of data in order to ensure the algorithms produce images of sufficiently high-quality. 

In this article, we propose to present an overview of recent advances in reconstruction algorithms for improving the performance of scientific CT systems - enabling faster, more accurate and novel imaging capabilities. 
The first part of the article will focus on model-based image reconstruction (MBIR) algorithms \cite{Bo641Text} that formulate the inversion as solving a high-dimensional optimization problem involving a data-fidelity term (forward model) and a regularization term. 
By accurately modeling the physics+noise statistics of the measurement and combining it with state-of-the art regularizers, we will illustrate how dramatic improvements are being made in the performance of scientific CT instruments used in the  materials sciences - electron CT \cite{GorisCompSenseET,leary2013compressed,VenkatHAADF13,VenkatBF15}, X-ray micro-CT \cite{AdityaICASSP14,AdityaTIMBIR,gursoy2015hyperspectral} and neutron CT \cite{VenkatLam17,kazantsev2017novel}.
We propose to categorize and identify the core novelty in these algorithms by the innovations in the design of forward model, regularizers \cite{ziabari2019physics} as well as summarize research in the development of fast algorithms that can leverage parallel/distributed computing platforms \cite{wang2017massively,marchesini2020sparse,wang2019consensus} to perform the optimization that are essential to making such methods available in practice to experimental scientists.  
In the last part of the article, we will present an overview of recent approaches using direct deep-learning based algorithms for improving scientific CT instruments. 
By direct deep-learning, we mean non-iterative neural-network-based algorithms that are typically designed to suppress different artifacts that occur in the context of challenging scientific CT data sets  \cite{venkatMLST20,pelt2018improving,yang2018low,liu2020tomogan}.
The key appeal of the direct deep-learning approaches is that they promise a inference time computational  complexity that is similar to the analytic approaches that are routinely used while offering the potential to obtain reconstruction quality that is competitive to the model-based approaches.  
We will start by identifying when such deep-learning methods are being considered in the context of scientific CT (for example to measure a sequence of samples, time-resolved CT etc.), followed by the challenges of availability of smaller 3D training data sets and the potential solution that involve smaller networks or various data augmentation techniques. 
Finally, we will highlight challenges that still exist in extending the use of such techniques for materials imaging.

\section*{Outline of Proposed Paper}

\subsection*{Introduction: CT for Materials Imaging}

\begin{itemize}
    \item Basics of CT and the broad categories of CT reconstruction algorithms  - analytic, iterative, model-based iterative and corresponding  deep-learning driven improvements of the analytic and MBIR categories \cite{mccann2017convolutional}. 
    \item Different instruments used to perform CT (for example: electron, X-rays, Neutron microscopes), the underlying challenges that cut across the different applications (such as mis-calibrations, non-linearity of models, low signal to noise ratio etc.) and typical analytic reconstruction methods.
\end{itemize}

\subsection*{Model-Based Image Reconstruction for Scientific CT}

\begin{itemize} 
\item The key-equation corresponding to MBIR approaches - formulating and minimizing a  cost-function consisting of two sets of terms. All subsequent details will be discussed in the context of this master equation with some mathematical details of the different forward model terms and regularizers that have been developed to deal with the sparse-view, noisy, limited-angle, mis-calibrated and non-linear measurement data. 
\item We will show images/visualizations of how MBIR methods have enabled higher quality 3D imaging for electron tomography (where we deal with low-dose, noisy, sparse +limited-angle data, non-linear forward models) \cite{GorisCompSenseET,VenkatHAADF13,VenkatBF15,migunov2015rapid}, synchrotron-based and neutron-based micro-CT (sparse-view, low signal-to-noise ratio data with outliers, other detector mis-calibration, and non-linear forward models) \cite{AdityaICASSP14,kazantsev2017novel}.
\item Present the emerging area of studying changes in materials at the sub-micron scale using time-resolved CT for which MBIR approaches have been critical in obtaining dramatic improvements in spatio-temporal resolution \cite{AdityaTIMBIR,zang2018space}. 
\item  Discuss the issue of the high computational complexity of MBIR methods and the efforts to accelerate the reconstruction using heterogeneous high-performance computing platforms \cite{wang2017massively,marchesini2020sparse,wang2019consensus}.  
\end{itemize}
%We will also discuss the key role open-source software \cite{gursoy2014tomopy,AstraGPU11,vanAarleASTRA16,wang2017massively} is playing to accelerate adoption of new algorithms for scientific CT. 
%The take home message of this section will be
%Conventional 3D CT  \cite{VenkatHAADF13,VenkatBF15,VenkatLam17,AdityaICASSP14,kazantsev2017novel}, time-resolved CT \cite{AdityaTIMBIR}. %Cite Sara Bals, Joost and others from the European groups. 
\subsection*{Direct Deep-Learning Algorithms for Scientific CT}
\begin{itemize}
    \item Present the general trend of using neural networks for CT reconstruction \cite{mccann2017convolutional} and the benefits of the non-iterative deep learning (DL) approaches for scientific CT. 
    \item Discuss when DL is applicable for scientific CT - sequence of similar samples, time-resolved CT, and for samples manufactured based on a computer aided drawing (CAD) model. Highlight the small data problem and the "3D" nature of the modality.
    \item Highlight and summarize recent research on adapting neural network techniques for (a) 3D CT based on a reference scan  \cite{yang2018low,anirudh2018lose,pelt2013fast,pelt2018improving,venkatMLST20,liu2020tomogan,ziabari2020IMECE}, and (b) time-resolved CT \cite{majee20194d} that have enabled dramatic acceleration in data acquisition (by up to an order of magnitude) while preserving reconstruction quality. 
\end{itemize}

\subsection*{Discussion}
\begin{itemize}
    \item Overall conclusion of using modern reconstruction algorithms to enable new capabilities for scientific CT instruments.         
    \item Important future research directions still need to be pursued to increase adoption of these modern techniques to scientific CT instruments - task driven choice of algorithm parameters, faster algorithms, modular and accessible software. 
    
\end{itemize}



